Probabilistic Circuits for Variational Inference in Discrete Graphical Models

Inference in discrete graphical models with variational methods is difficult because of the inability to re-parameterize gradients of the Evidence Lower Bound (ELBO). Many sampling-based methods have been proposed for estimating these gradients, but they suffer from high bias or variance. In this paper, we propose a new approach that leverages the tractability of probabilistic circuit models, such as Sum Product Networks (SPN), to compute ELBO gradients exactly (without sampling) for a certain class of densities. In particular, we show that selective-SPNs are suitable as an expressive variational distribution, and prove that when the log-density of the target model is a polynomial the corresponding ELBO can be computed analytically. To scale to graphical models with thousands of variables, we develop an efficient and effective construction of selective-SPNs with size $O(kn)$, where $n$ is the number of variables and $k$ is an adjustable hyperparameter. We demonstrate our approach on three types of graphical models -- Ising models, Latent Dirichlet Allocation, and factor graphs from the UAI Inference Competition. Selective-SPNs give a better lower bound than mean-field and structured mean-field, and is competitive with approximations that do not provide a lower bound, such as Loopy Belief Propagation and Tree-Reweighted Belief Propagation. Our results show that probabilistic circuits are promising tools for variational inference in discrete graphical models as they combine tractability and expressivity.

==> comp_graph.tex <==
\tikzstyle{inputNode}=[circle,minimum size=20pt,inner sep=0pt]
\tikzstyle{stateTransition}=[-stealth, thick]


\begin{figure}
\centering
\begin{tikzpicture}[scale=0.8]

    \pgfmathsetmacro{\yd}{1.25}
    \pgfmathsetmacro{\xd}{1.5}

	\node[inputNode] (phi) at (0*\xd, 0*\yd) {\(\phi\)};
	
	\node[inputNode] (thetac) at (2*\xd, 2*\yd) {\(\theta\)};
	\node[inputNode] (zc) at (2*\xd, 1*\yd) {\(\z_c\)};
	\node[inputNode] (h) at (4*\xd, 1*\yd) {\(h_\theta\)};
	
	\node[inputNode] (zd) at (2*\xd, -1*\yd) {\(\z_d\)};
	\node[inputNode] (g) at (4*\xd, -1*\yd) {\(g_{\lambda}\)};
	
	\node[inputNode] (x) at (6*\xd, -1*\yd) {\(\tilde{\x}\)};

 	\draw[stateTransition] (phi) to node[midway, sloped, above] {\(q_{\phi}(\z_c|\x)\)} (zc);
 	\draw[stateTransition] (phi) to node[midway, sloped, above] {\(q_{\phi}(\z_d|\x)\)} (zd);
 	

 	\draw[stateTransition] (zc) to (h);
 	\draw[stateTransition] (thetac) to (h);
 	%\draw[stateTransition, dashed] (h) to (x);
 	
 	\draw[stateTransition] (h) to node[midway, left] {\(\lambda\)} (g);
 	
 	\draw[stateTransition] (zd) to (g);
 	\draw[stateTransition] (g) to (x);

    
    %\draw[stateTransition] (zc) to[out=-20,in=-140] node[midway, sloped, above] {\(p(\x|\z_c)\)} (x);

\end{tikzpicture}

\caption{The computation graph of the VAE. First we encode a given \(\x\) into Gaussian distributions over \(\z_c\) and Bernoulli distributions over \(\z_d\). We sample only the continuous latent variables \(\z_c\), and marginalize out the discrete latent variables \(\z_d\), which is possible since \(g_\lambda\) is a probabilistic circuit.
}
\label{fig:compgraph}

\end{figure}

==> tikzlibraryspn.code.tex <==
\usetikzlibrary{chains}
%\usetikzlibrary{arrows}
\usepackage{pgfplots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

% sum node style
\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=16pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

% product node style
\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=16pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

% \sumnode [tikz-options] {sum node name} 
\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

% \prodnode [tikz-options] {product node name} 
\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {$\times$};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

% \maxnode [tikz-options] {max node name} 
\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

% \emptynode [tikz-options] {generic node name}
\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=16pt, font=\small, #1] (#2) {#3};
}

\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=16pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=16pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

